Gene network robustness as a multivariate character

Robustness to genetic or environmental disturbances is often considered as a key property of living systems. Yet, in spite of being discussed since the 1950s, how robustness emerges from the complexity of genetic architectures and how it evolves still remains unclear. In particular, whether or not robustness is independent to various sources of perturbations conditions the range of adaptive scenarios that can be considered. For instance, selection for robustness to heritable mutations is likely to be modest and indirect, and its evolution might result from indirect selection on a pleiotropically-related character (e.g., homeostasis). Here, I propose to treat various robustness measurements as quantitative characters, and study theoretically, by individual-based simulations, their propensity to evolve independently. Based on a simple evolutionary model of a gene regulatory network, I showed that five measurements of the robustness of gene expression to genetic or non-genetic disturbances were substantially correlated. Yet, robustness was mutationally variable in several dimensions, and robustness components could evolve differentially under direct selection pressure. Therefore, the fact that the sensitivity of gene expression to mutations and environmental factors rely on the same gene networks does not preclude distinct evolutionary histories of robustness components. This article has been peer-reviewed and recommended by Peer Community In Evolutionary Biology Posted: 30th March 2022 (https://doi.org/10.24072/pci.evolbiol.100138)

==> preambule.tex <==
%%%%%%%%%%TO FORMAT A PREPRINT%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[top=7cm,bottom=2.5cm,headheight=120pt,headsep=15pt,left=6cm,right=1.5cm,marginparwidth=4.2cm,marginparsep=0.5cm]{geometry}


\usepackage{marginnote}
\reversemarginpar  % sets margin notes to the left
\usepackage{lipsum} % Required to insert dummy text
\usepackage{calc}
\usepackage{siunitx}
\usepackage{lineno}
%\usepackage[none]{hyphenat} % use only if there is a problem
% Use Unicode characters
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
% Clean citations with biblatex
\usepackage[
backend=biber,
natbib=true,
sortcites=true,
defernumbers=true,
style=authoryear,
citestyle=authoryear-comp,
maxnames=99,
maxcitenames=2,
giveninits=true,
terseinits=true,
url=false
]{biblatex}
\DeclareNameAlias{default}{family-given}
\renewcommand*{\revsdnamepunct}{} % no comma between family and given names
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}} % remove 'In:' before journal name
\DeclareFieldFormat[article]{pages}{#1} % remove pp.
\AtEveryBibitem{\ifentrytype{article}{\clearfield{number}}{}} % don't print issue numbers
\DeclareFieldFormat[article, inbook, incollection, inproceedings, misc, thesis, unpublished]{title}{#1} % title without quotes
\usepackage{csquotes}
\RequirePackage[english]{babel} % must be called after biblatex
\addbibresource{sample.bib}
\DeclareBibliographyCategory{ignore}
\addtocategory{ignore}{recommendation} % adding recommendation to 'ignore' category so that it does not appear in the References
% Clickable references. Use \url{www.example.com} or \href{www.example.com}{description} to add a clicky url
\usepackage{nameref}
\usepackage[pdfborder={0 0 0}]{hyperref}  % sets link border to white
\urlstyle{same}

\if{\PCI=cneuro}{\newcommand{\logo}{logo_pour_PDF_evolbiol.png}}\fi


%logo_pour_PDF_cneuro.png
%small_logo_pour_PDF_cneuro.png
%Peer Community In Circuit Neuroscience


% Include figures
\usepackage{graphbox}  % loads graphicx ppackage with extended options for vertical alignment of figures
% Line numbers
%\usepackage[right]{lineno}
% Improve typesetting in LaTex
\usepackage{microtype}
\DisableLigatures[f]{encoding = *, family = * }
% Text layout and font (Open Sans)
\setlength{\parindent}{0.4cm}
\linespread{1.2}
\RequirePackage[default,scale=0.90]{opensans}
% Defining document colors
\usepackage{xcolor}
\definecolor{darkgray}{HTML}{808080}
\definecolor{mediumgray}{HTML}{6D6E70}
\definecolor{ligthgray}{HTML}{d9d9d9}
\definecolor{pciblue}{HTML}{74adca}
\definecolor{opengreen}{HTML}{77933c}
% Use adjustwidth environment to exceed text width
\usepackage{changepage}
% Adjust caption style
\usepackage[aboveskip=1pt,labelfont=bf,labelsep=period,singlelinecheck=off]{caption}

% Headers and footers
\usepackage{fancyhdr}  % custom headers/footers
\usepackage{lastpage}  % number of page in the document
\pagestyle{fancy}  % enables customization of headers/footers
\fancyhfoffset[L]{4.5cm}  % offsets header and footer to the left to include margin
\renewcommand{\headrulewidth}{\ifnum\thepage=1 0.5pt \else 0pt \fi} % header ruler only on first page
\renewcommand{\footrulewidth}{0.5pt}
% full logo on first page, then small logo on subsequent pages 

\lhead{\ifnum\thepage=1 \includegraphics[width=13.5cm]{\logo} \else \includegraphics[width=5cm]{small_logo_pour_PDF_cneuro.png} \fi}  

\chead{}
\rhead{}

\newcommand{\DOIlink}{\href{https://dx.doi.org/\DOI}{\DOI}}

\newcommand{\DOIrecommendationlink}{\href{https://dx.doi.org/\DOIrecommendation}{\DOIrecommendation}}

\lfoot{\scriptsize \textsc{\color{mediumgray}\PCI}}

\cfoot{}
\rfoot{\scriptsize\thepage\space of\space\pageref{LastPage}}


\newcommand{\PCI}{Peer Community In Circuit Neuroscience}


\newcommand{\beginingpreprint}{
\vspace*{0.5cm}
\begin{flushleft}
\baselineskip=30pt
%\marginpar{\includegraphics[align=c,width=0.5cm]{OAlogogreen.png} \space %\large\textbf{\color{opengreen}Open Access}\\
%\\
%\large\textnormal{\color{opengreen}PREPRINT}}
% Margin information
\marginpar{
\large\textnormal{\color{pciblue}\\RESEARCH ARTICLE}\\
\vspace*{0.5pt}
\\
\includegraphics[align=c,width=0.5cm]{OAlogoblue.png} \space \large\textbf{\color{pciblue}Open Access}\\
\\
\includegraphics[align=c,width=0.5cm]{o_peerreview.png} \space \large\textbf{\color{pciblue}Open Peer-Review}\\
\\
\includegraphics[align=c,width=0.5cm]{o_data3.png} \space \large\textbf{\color{pciblue}Open Data}\\
\\
\includegraphics[align=c,width=0.5cm]{o_script3.png} \space \large\textbf{\color{pciblue}Open Code}\\
\\
\\
\\
\\
\raggedright
%\vspace*{3.25cm}
\scriptsize\textbf{Cite as:}\space
\citeas\\
\vspace*{0.5cm}
\textbf{Posted:} \datepub\\
\vspace*{0.5cm}
\textbf{Recommender:}\\
\recommender\\
\vspace*{0.5cm}
\textbf{Reviewers:}\\
\reviewers\\
\vspace*{0.5cm}
\textbf{Correspondence:}\\
\href{mailto:\email}{\email}\\


}
{\Huge
\fontseries{sb}\selectfont{\preprinttitle}}
\end{flushleft}
\vspace*{0.25cm}
\begin{flushleft}
%\marginpar{


%\marginnote{
%\raggedright
%\vspace*{3.25cm}
%\scriptsize\textbf{Cite as:}\space
%\fullcite{preprint}\\
%\vspace*{0.5cm}
%\textbf{Published:} \datepub\\
%\vspace*{0.5cm}
%\textbf{Recommender:}\\
%\recommender\\
%\vspace*{0.5cm}
%\textbf{Reviewers:}\\
%\reviewers\\
%\vspace*{0.5cm}
%\textbf{Correspondence:}\\
%\href{mailto:\email}{\email}\\
%\vspace*{0.5cm} 
%\vspace*{3cm}
%\vspace*{0.2cm}
%}[0.8cm]


\Large
\listauthors
\end{flushleft}
\bigskip
{\raggedright
\listinstitutions}
% Recommended preprint box
\begin{flushleft}
%\noindent
\fcolorbox{lightgray}{lightgray}{
\parbox{\textwidth - 2\fboxsep}{
\centering\large{\fontseries{sb}\selectfont{This article has been peer-reviewed and recommended by\\
\emph{\PCI}}}\\
%\raggedright\large{\fontseries{sb}\selectfont{An article peer-reviewed and recommended by \emph{\PCI}, edited by \recommender \space on the basis of the reviews by \reviewers \space (DOI: \DOIrecommendationlink)}}\\
%\small \fullcite{preprint}
}}
\end{flushleft}
\vspace*{0.5cm}
\fcolorbox{pciblue}{pciblue}{
\parbox{\textwidth - 2\fboxsep}{
\vspace{0.25cm}
\textbf{\large{\textsc{Abstract}}}\\
\preprintabstract\\

\footnotesize{\textbf{\emph{Keywords: }}\preprintkeywords}
\vspace{0.25cm}}
}
}




